Intersection of paraboloids and application to Minkowski-type problems

In this article, we study the intersection (or union) of the convex hull of N confocal paraboloids (or ellipsoids) of revolution. This study is motivated by a Minkowski-type problem arising in geometric optics. We show that in each of the four cases, the combinatorics is given by the intersection of a power diagram with the unit sphere. We prove the complexity is O(N) for the intersection of paraboloids and Omega(N^2) for the intersection and the union of ellipsoids. We provide an algorithm to compute these intersections using the exact geometric computation paradigm. This algorithm is optimal in the case of the intersection of ellipsoids and is used to solve numerically the far-field reflector problem.

==> app.tex <==
\appendix
\section{Proofs}

%---------------------------------- SANS LA GENERICITÉ
%\begin{proof}[Proof of Proposition~\ref{prop:comp}]
%We take a family of $N$ real numbers $(t_i)_{1\leq i \leq N}$. For every $i\in\{1,\hdots,N\}$, we put $\lambda_i=1$ and $y_i=\varphi(t_i)$ , where the map $\varphi:\Rsp\to \Rsp^3$ defined by $\varphi(t)=(\frac{t^2-1}{1+t^2},\frac{2t}{1+t^2},0)$ is a parameterization of the equator  $\Sph^2 \cap \{z=0\}$ from which we removed the point $(1,0,0)$. The family of paraboloids $(P(y_i,\lambda))_{1\leq i \leq N}$ is such that every cell $\PI_{Y}^\lambda(y_i)$ is delimited by two half great circles between the two poles, each of these half circles being shared by two cells.
%There exists a cycle with the $N$ vertices of $\{y_1,\hdots,y_{N}\}$ in the dual of the paraboloid intersection diagram. Finding this cycle  then amounts to sorting the values $(t_i)_{1\leq i \leq N}$. The conclusion holds from the fact that a sorting algorithm has a complexity $\Omega(N\log(N))$.
%\end{proof}


